Dynamic Distillation Network for Cross-Domain Few-Shot Recognition with Unlabeled Data

Most existing works in few-shot learning rely on meta-learning the network on a large base dataset which is typically from the same domain as the target dataset. We tackle the problem of cross-domain few-shot learning where there is a large shift between the base and target domain. The problem of cross-domain few-shot recognition with unlabeled target data is largely unaddressed in the literature. STARTUP was the first method that tackles this problem using self-training. However, it uses a fixed teacher pretrained on a labeled base dataset to create soft labels for the unlabeled target samples. As the base dataset and unlabeled dataset are from different domains, projecting the target images in the class-domain of the base dataset with a fixed pretrained model might be sub-optimal. We propose a simple dynamic distillation-based approach to facilitate unlabeled images from the novel/base dataset. We impose consistency regularization by calculating predictions from the weakly-augmented versions of the unlabeled images from a teacher network and matching it with the strongly augmented versions of the same images from a student network. The parameters of the teacher network are updated as exponential moving average of the parameters of the student network. We show that the proposed network learns representation that can be easily adapted to the target domain even though it has not been trained with target-specific classes during the pretraining phase. Our model outperforms the current state-of-the art method by 4.4% for 1-shot and 3.6% for 5-shot classification in the BSCD-FSL benchmark, and also shows competitive performance on traditional in-domain few-shot learning task.

==> NeurIPS2021/Tables/main_tbl/ablation_different_datasets.tex <==
\begin{tabular}{llllll}
\toprule
{} &                   EuroSAT &               CropDisease &                    ChestX &                      ISIC                        \\
\midrule
Ours-EuroSAT     &  88.26{\small $\pm$.46} &  89.20{\small $\pm$.56} &  25.11{\small $\pm$.42} &  47.11{\small $\pm$.61} \\
Ours-CropDisease &  82.04{\small $\pm$.61} &  95.78{\small $\pm$.34} &  25.63{\small $\pm$.44} &  47.44{\small $\pm$.61}  \\
Ours-ChestX      &  79.81{\small $\pm$.62} &  89.51{\small $\pm$.54} &  27.82{\small $\pm$.44} &  44.17{\small $\pm$.58}  \\
Ours-ISIC        &  80.71{\small $\pm$.64} &  87.87{\small $\pm$.60} &  26.58{\small $\pm$.43} &  48.26{\small $\pm$.56} \\
Ours-all & 83.87{\small $\pm$.54} &  87.40{\small $\pm$.56} &  28.71{\small $\pm$.46} &  46.63{\small $\pm$.59} \\
\bottomrule
\end{tabular}


==> NeurIPS2021/Tables/main_tbl/resnet10_miniImageNet_20shot_s.tex <==
\begin{tabular}{lllll}
\toprule
{} &                 EuroSAT &             CropDisease &                    ISIC &                  ChestX \\
\midrule
protonet             &  82.53{\small $\pm$.55} &  89.34{\small $\pm$.48} &  50.79{\small $\pm$.57} &  28.96{\small $\pm$.43} \\
matchingnet          &  76.22{\small $\pm$.57} &  76.66{\small $\pm$.73} &  43.24{\small $\pm$.53} &  26.17{\small $\pm$.38} \\
ce                   &  88.70{\small $\pm$.45} &  96.04{\small $\pm$.26} &  56.96{\small $\pm$.54} &  31.91{\small $\pm$.47} \\
simclr               &  88.42{\small $\pm$.47} &  91.29{\small $\pm$.42} &  52.82{\small $\pm$.52} &  33.30{\small $\pm$.43} \\
simclr-u             &  89.62{\small $\pm$.42} &  95.57{\small $\pm$.30} &  50.96{\small $\pm$.52} &  36.52{\small $\pm$.51} \\
startup              &  90.34{\small $\pm$.44} &  97.06{\small $\pm$.24} &  56.99{\small $\pm$.56} &  33.19{\small $\pm$.46} \\
ce-simclr            &  92.31{\small $\pm$.33} &  96.70{\small $\pm$.27} &  55.86{\small $\pm$.52} &  37.51{\small $\pm$.53} \\
ce-distill-self-sgd  &  93.26{\small $\pm$.32} &  98.17{\small $\pm$.18} &  58.89{\small $\pm$.56} &  35.37{\small $\pm$.48} \\
ce-distill-fixed-sgd &  91.64{\small $\pm$.39} &  97.26{\small $\pm$.22} &  60.00{\small $\pm$.57} &  34.12{\small $\pm$.47} \\
ce-distill-ema-sgd   &  92.95{\small $\pm$.33} &  98.07{\small $\pm$.19} &  58.58{\small $\pm$.57} &  35.89{\small $\pm$nan} \\
\bottomrule
\end{tabular}


==> NeurIPS2021/Tables/main_tbl/resnet10_miniImageNet_50shot_s.tex <==
\begin{tabular}{lllll}
\toprule
{} &                 EuroSAT &             CropDisease &                    ISIC &                  ChestX \\
\midrule
protonet             &  84.76{\small $\pm$.51} &  91.35{\small $\pm$.42} &  52.15{\small $\pm$.53} &  31.34{\small $\pm$.44} \\
matchingnet          &  43.37{\small $\pm$.53} &  49.11{\small $\pm$.66} &  28.61{\small $\pm$.40} &  21.36{\small $\pm$.29} \\
ce                   &  91.17{\small $\pm$.36} &  97.59{\small $\pm$nan} &  63.15{\small $\pm$nan} &  35.35{\small $\pm$nan} \\
simclr               &  91.18{\small $\pm$.37} &  94.18{\small $\pm$.34} &  58.73{\small $\pm$.49} &  38.14{\small $\pm$.46} \\
simclr-u             &  91.88{\small $\pm$.33} &  97.28{\small $\pm$.24} &  57.13{\small $\pm$nan} &  40.26{\small $\pm$nan} \\
startup              &  92.62{\small $\pm$nan} &  98.33{\small $\pm$nan} &  63.56{\small $\pm$nan} &  35.67{\small $\pm$nan} \\
ce-simclr            &  93.92{\small $\pm$.28} &  98.05{\small $\pm$.21} &  61.40{\small $\pm$.53} &  40.90{\small $\pm$nan} \\
ce-distill-self-sgd  &  94.76{\small $\pm$.25} &  98.86{\small $\pm$.14} &  64.26{\small $\pm$nan} &  38.71{\small $\pm$nan} \\
ce-distill-fixed-sgd &  93.34{\small $\pm$.31} &  98.42{\small $\pm$.16} &  64.99{\small $\pm$nan} &  38.14{\small $\pm$nan} \\
ce-distill-ema-sgd   &  94.38{\small $\pm$.27} &  98.84{\small $\pm$.15} &  63.82{\small $\pm$.57} &  39.42{\small $\pm$nan} \\
\bottomrule
\end{tabular}


==> NeurIPS2021/Tables/main_tbl/resnet18_miniImageNet_20shot_s.tex <==
\begin{tabular}{lllll}
\toprule
{} &                 EuroSAT &             CropDisease &                    ISIC &                  ChestX \\
\midrule
protonet             &  83.31{\small $\pm$.56} &  89.52{\small $\pm$.45} &  49.13{\small $\pm$.58} &  28.75{\small $\pm$.43} \\
matchingnet          &  73.81{\small $\pm$.65} &  79.45{\small $\pm$.70} &  36.71{\small $\pm$.46} &  26.15{\small $\pm$.40} \\
ce                   &  87.60{\small $\pm$.47} &  95.17{\small $\pm$.30} &  56.13{\small $\pm$.54} &  31.42{\small $\pm$.47} \\
simclr               &  88.40{\small $\pm$.46} &  91.34{\small $\pm$.42} &  52.36{\small $\pm$.51} &  33.68{\small $\pm$.43} \\
simclr-u             &  90.34{\small $\pm$.41} &  95.75{\small $\pm$.32} &  49.83{\small $\pm$.52} &  35.69{\small $\pm$.50} \\
startup              &  90.47{\small $\pm$.45} &  96.90{\small $\pm$.26} &  56.40{\small $\pm$.57} &  31.16{\small $\pm$.46} \\
ce-simclr            &  93.19{\small $\pm$.32} &  96.42{\small $\pm$.28} &  54.84{\small $\pm$.54} &  36.45{\small $\pm$.49} \\
ce-distill-self-sgd  &  90.96{\small $\pm$.41} &  96.16{\small $\pm$.26} &  57.86{\small $\pm$.55} &  32.53{\small $\pm$.44} \\
ce-distill-fixed-sgd &  90.60{\small $\pm$.42} &  95.55{\small $\pm$.28} &  58.23{\small $\pm$.54} &  33.40{\small $\pm$.45} \\
ce-distill-ema-sgd   &  92.04{\small $\pm$.37} &  96.55{\small $\pm$.25} &  57.82{\small $\pm$.57} &  33.16{\small $\pm$.45} \\
\bottomrule
\end{tabular}


==> NeurIPS2021/Tables/main_tbl/resnet18_miniImageNet_50shot_s.tex <==
\begin{tabular}{lllll}
\toprule
{} &                 EuroSAT &             CropDisease &                    ISIC &                  ChestX \\
\midrule
protonet             &  85.05{\small $\pm$.49} &  91.73{\small $\pm$.41} &  52.45{\small $\pm$.53} &  30.91{\small $\pm$.42} \\
matchingnet          &  58.54{\small $\pm$.61} &  64.02{\small $\pm$.81} &  38.04{\small $\pm$.46} &  23.27{\small $\pm$.36} \\
ce                   &  90.31{\small $\pm$.40} &  96.97{\small $\pm$.24} &  61.47{\small $\pm$nan} &  34.71{\small $\pm$nan} \\
simclr               &  91.38{\small $\pm$.36} &  94.30{\small $\pm$nan} &  57.97{\small $\pm$nan} &  37.78{\small $\pm$.48} \\
simclr-u             &  92.25{\small $\pm$nan} &  97.32{\small $\pm$.23} &  55.41{\small $\pm$nan} &  38.46{\small $\pm$nan} \\
startup              &  92.52{\small $\pm$nan} &  98.08{\small $\pm$.20} &  62.20{\small $\pm$nan} &  33.99{\small $\pm$nan} \\
ce-simclr            &  94.40{\small $\pm$.26} &  97.80{\small $\pm$nan} &  59.52{\small $\pm$nan} &  39.15{\small $\pm$nan} \\
ce-distill-self-sgd  &  92.55{\small $\pm$.33} &  97.69{\small $\pm$.21} &  63.57{\small $\pm$.57} &  36.55{\small $\pm$nan} \\
ce-distill-fixed-sgd &  92.51{\small $\pm$.35} &  97.32{\small $\pm$.22} &  63.45{\small $\pm$.55} &  37.33{\small $\pm$.47} \\
ce-distill-ema-sgd   &  93.46{\small $\pm$.30} &  97.85{\small $\pm$.19} &  62.80{\small $\pm$nan} &  37.36{\small $\pm$.46} \\
\bottomrule
\end{tabular}


==> NeurIPS2021/Tables/main_tbl/resnet18_miniImageNet_5shot_s.tex <==
\begin{tabular}{lllll}
\toprule
{} &                 EuroSAT &             CropDisease &                    ISIC &                  ChestX \\
\midrule
protonet             &  75.84{\small $\pm$.69} &  79.91{\small $\pm$.72} &  43.00{\small $\pm$.60} &  24.33{\small $\pm$.42} \\
matchingnet          &  69.41{\small $\pm$.79} &  61.79{\small $\pm$.88} &  35.03{\small $\pm$.56} &  22.92{\small $\pm$.39} \\
ce                   &  79.66{\small $\pm$.66} &  88.23{\small $\pm$.55} &  45.37{\small $\pm$.58} &  25.33{\small $\pm$.44} \\
simclr               &  81.01{\small $\pm$.65} &  83.10{\small $\pm$.61} &  43.59{\small $\pm$.56} &  27.13{\small $\pm$.44} \\
simclr-u             &  84.40{\small $\pm$.54} &  89.98{\small $\pm$.55} &  42.50{\small $\pm$.54} &  29.84{\small $\pm$.49} \\
startup              &  84.88{\small $\pm$.59} &  92.44{\small $\pm$.47} &  46.58{\small $\pm$.62} &  25.71{\small $\pm$.44} \\
ce-simclr            &  87.26{\small $\pm$.47} &  91.07{\small $\pm$.52} &  45.84{\small $\pm$.54} &  29.89{\small $\pm$.47} \\
ce-distill-self-sgd  &  85.86{\small $\pm$.53} &  91.21{\small $\pm$.45} &  47.48{\small $\pm$.61} &  26.14{\small $\pm$.45} \\
ce-distill-fixed-sgd &  85.63{\small $\pm$.58} &  89.87{\small $\pm$.51} &  48.06{\small $\pm$.58} &  26.35{\small $\pm$.45} \\
ce-distill-ema-sgd   &  87.43{\small $\pm$.52} &  92.23{\small $\pm$.43} &  48.22{\small $\pm$.59} &  26.62{\small $\pm$.44} \\
\bottomrule
\end{tabular}


==> NeurIPS2021/Tables/main_tbl/resnet18_tieredImageNet_1shot_s.tex <==
\begin{tabular}{lllll}
\toprule
{} &                 EuroSAT &             CropDisease &                    ISIC &                  ChestX \\
\midrule
ce                   &  58.07{\small $\pm$.86} &  69.94{\small $\pm$.87} &  29.76{\small $\pm$.55} &  22.46{\small $\pm$.41} \\
simclr               &  62.14{\small $\pm$.89} &  62.45{\small $\pm$.90} &  31.03{\small $\pm$.55} &  22.28{\small $\pm$.40} \\
simclr-u             &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} \\
startup              &  64.32{\small $\pm$.87} &  70.09{\small $\pm$.86} &  29.73{\small $\pm$.51} &  22.10{\small $\pm$.40} \\
ce-simclr            &  58.08{\small $\pm$.83} &  71.25{\small $\pm$.89} &  31.71{\small $\pm$.55} &  23.81{\small $\pm$.46} \\
ce-distill-self-sgd  &  74.00{\small $\pm$.76} &  85.34{\small $\pm$.76} &  34.78{\small $\pm$.60} &  22.49{\small $\pm$.40} \\
ce-distill-fixed-sgd &  68.74{\small $\pm$.79} &  80.04{\small $\pm$.79} &  35.07{\small $\pm$.62} &  23.18{\small $\pm$.43} \\
ce-distill-ema-sgd   &  72.15{\small $\pm$.75} &  84.41{\small $\pm$.75} &  33.87{\small $\pm$.56} &  22.70{\small $\pm$.42} \\
\bottomrule
\end{tabular}


==> NeurIPS2021/Tables/main_tbl/resnet18_tieredImageNet_20shot_s.tex <==
\begin{tabular}{lllll}
\toprule
{} &                 EuroSAT &             CropDisease &                    ISIC &                  ChestX \\
\midrule
ce                   &  88.90{\small $\pm$.40} &  95.62{\small $\pm$.31} &  51.49{\small $\pm$.53} &  32.34{\small $\pm$.45} \\
simclr               &  89.72{\small $\pm$.43} &  92.13{\small $\pm$.41} &  52.66{\small $\pm$.52} &  32.08{\small $\pm$.46} \\
simclr-u             &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} \\
startup              &  91.63{\small $\pm$.36} &  96.05{\small $\pm$.30} &  53.90{\small $\pm$.55} &  31.85{\small $\pm$.46} \\
ce-simclr            &  93.01{\small $\pm$.31} &  96.60{\small $\pm$.27} &  55.01{\small $\pm$.53} &  37.59{\small $\pm$.51} \\
ce-distill-self-sgd  &  94.78{\small $\pm$.26} &  98.32{\small $\pm$.18} &  56.93{\small $\pm$.53} &  33.39{\small $\pm$.48} \\
ce-distill-fixed-sgd &  94.64{\small $\pm$.27} &  97.53{\small $\pm$.23} &  57.89{\small $\pm$.54} &  34.82{\small $\pm$.49} \\
ce-distill-ema-sgd   &  94.20{\small $\pm$.28} &  98.33{\small $\pm$.19} &  56.50{\small $\pm$.54} &  34.58{\small $\pm$.47} \\
\bottomrule
\end{tabular}


==> NeurIPS2021/Tables/main_tbl/resnet18_tieredImageNet_50shot_s.tex <==
\begin{tabular}{lllll}
\toprule
{} &                 EuroSAT &             CropDisease &                    ISIC &                  ChestX \\
\midrule
ce                   &  91.27{\small $\pm$.31} &  97.33{\small $\pm$.23} &  57.21{\small $\pm$.54} &  35.47{\small $\pm$nan} \\
simclr               &  92.67{\small $\pm$.31} &  94.71{\small $\pm$.33} &  58.57{\small $\pm$nan} &  35.40{\small $\pm$nan} \\
simclr-u             &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} \\
startup              &  93.65{\small $\pm$nan} &  97.68{\small $\pm$.22} &  59.03{\small $\pm$.55} &  35.08{\small $\pm$.46} \\
ce-simclr            &  94.51{\small $\pm$.25} &  97.84{\small $\pm$.22} &  60.00{\small $\pm$.54} &  41.24{\small $\pm$.52} \\
ce-distill-self-sgd  &  95.77{\small $\pm$.22} &  98.83{\small $\pm$.15} &  61.92{\small $\pm$.55} &  36.22{\small $\pm$nan} \\
ce-distill-fixed-sgd &  95.85{\small $\pm$.23} &  98.31{\small $\pm$.18} &  62.50{\small $\pm$.54} &  38.09{\small $\pm$.50} \\
ce-distill-ema-sgd   &  95.52{\small $\pm$.23} &  98.96{\small $\pm$.14} &  61.98{\small $\pm$.54} &  37.94{\small $\pm$nan} \\
\bottomrule
\end{tabular}


==> NeurIPS2021/Tables/main_tbl/resnet34_tieredImageNet_1shot_s.tex <==
\begin{tabular}{lllll}
\toprule
{} &                 EuroSAT &             CropDisease &                    ISIC &                  ChestX \\
\midrule
ce                   &  57.83{\small $\pm$.89} &  66.40{\small $\pm$.89} &  28.66{\small $\pm$.52} &  22.17{\small $\pm$.41} \\
simclr               &  63.70{\small $\pm$.93} &  64.31{\small $\pm$.94} &  30.40{\small $\pm$.53} &  22.47{\small $\pm$.42} \\
simclr-u             &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} \\
startup              &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} \\
ce-simclr            &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} \\
ce-distill-self-sgd  &  72.55{\small $\pm$.75} &  85.69{\small $\pm$.70} &  34.16{\small $\pm$.56} &  22.55{\small $\pm$.41} \\
ce-distill-fixed-sgd &  68.48{\small $\pm$.80} &  80.57{\small $\pm$.78} &  33.13{\small $\pm$.59} &  23.13{\small $\pm$.43} \\
ce-distill-ema-sgd   &  72.14{\small $\pm$.79} &  84.34{\small $\pm$.74} &  33.99{\small $\pm$.58} &  23.98{\small $\pm$.44} \\
\bottomrule
\end{tabular}


==> NeurIPS2021/Tables/main_tbl/resnet34_tieredImageNet_20shot_s.tex <==
\begin{tabular}{lllll}
\toprule
{} &                 EuroSAT &             CropDisease &                    ISIC &                  ChestX \\
\midrule
ce                   &  88.99{\small $\pm$.42} &  94.83{\small $\pm$.33} &  50.60{\small $\pm$.52} &  31.06{\small $\pm$.45} \\
simclr               &  89.62{\small $\pm$.44} &  92.72{\small $\pm$.41} &  50.84{\small $\pm$.52} &  31.71{\small $\pm$.46} \\
simclr-u             &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} \\
startup              &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} \\
ce-simclr            &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} \\
ce-distill-self-sgd  &  94.81{\small $\pm$.26} &  98.26{\small $\pm$.18} &  58.14{\small $\pm$.54} &  33.76{\small $\pm$.48} \\
ce-distill-fixed-sgd &  94.16{\small $\pm$.30} &  97.52{\small $\pm$.23} &  55.47{\small $\pm$.53} &  35.79{\small $\pm$.49} \\
ce-distill-ema-sgd   &  94.72{\small $\pm$.27} &  98.36{\small $\pm$.17} &  56.59{\small $\pm$.55} &  35.55{\small $\pm$.51} \\
\bottomrule
\end{tabular}


==> NeurIPS2021/Tables/main_tbl/resnet34_tieredImageNet_50shot_s.tex <==
\begin{tabular}{lllll}
\toprule
{} &                 EuroSAT &             CropDisease &                    ISIC &                  ChestX \\
\midrule
ce                   &  91.17{\small $\pm$.34} &  96.82{\small $\pm$.25} &  55.98{\small $\pm$.54} &  34.69{\small $\pm$.45} \\
simclr               &  92.54{\small $\pm$.32} &  95.53{\small $\pm$.32} &  57.17{\small $\pm$nan} &  35.36{\small $\pm$nan} \\
simclr-u             &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} \\
startup              &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} \\
ce-simclr            &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} \\
ce-distill-self-sgd  &  95.98{\small $\pm$.22} &  98.84{\small $\pm$.14} &  63.16{\small $\pm$.55} &  37.25{\small $\pm$.49} \\
ce-distill-fixed-sgd &  95.30{\small $\pm$.24} &  98.35{\small $\pm$.17} &  59.34{\small $\pm$.53} &  38.92{\small $\pm$.49} \\
ce-distill-ema-sgd   &  95.93{\small $\pm$.21} &  98.94{\small $\pm$.13} &  61.06{\small $\pm$.55} &  38.89{\small $\pm$.49} \\
\bottomrule
\end{tabular}


==> NeurIPS2021/Tables/main_tbl/resnet34_tieredImageNet_5shot_s.tex <==
\begin{tabular}{lllll}
\toprule
{} &                 EuroSAT &             CropDisease &                    ISIC &                  ChestX \\
\midrule
ce                   &  81.44{\small $\pm$.55} &  88.12{\small $\pm$.53} &  40.07{\small $\pm$.55} &  25.68{\small $\pm$.43} \\
simclr               &  82.09{\small $\pm$.62} &  84.91{\small $\pm$.63} &  41.57{\small $\pm$.56} &  26.04{\small $\pm$.42} \\
simclr-u             &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} \\
startup              &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} \\
ce-simclr            &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} &    nan{\small $\pm$nan} \\
ce-distill-self-sgd  &  90.57{\small $\pm$.38} &  96.19{\small $\pm$.33} &  48.28{\small $\pm$.59} &  27.14{\small $\pm$.46} \\
ce-distill-fixed-sgd &  88.69{\small $\pm$.46} &  94.45{\small $\pm$.38} &  46.68{\small $\pm$.56} &  28.50{\small $\pm$.48} \\
ce-distill-ema-sgd   &  90.16{\small $\pm$.40} &  96.01{\small $\pm$.33} &  47.50{\small $\pm$.56} &  29.56{\small $\pm$.49} \\
\bottomrule
\end{tabular}


==> NeurIPS2021/Tables/main_tbl/results_res10.tex <==
\begin{tabular}{lllll | llll}
\hline
\toprule
{} & \multicolumn{4}{c}{1-shot} &  \multicolumn{4}{c}{5-shot} \\
\cline{2-5}\cline{6-9}
\noalign{\smallskip} 
{Model} &                 EuroSAT &             CropDisease &                    ISIC &                  ChestX &                 EuroSAT &             CropDisease &                    ISIC &                  ChestX \\
\midrule
MAML$^*$ & -&-&-&-& 71.70{\small $\pm$.72} & 78.05{\small $\pm$.70} & 40.13{\small $\pm$.58}  &   23.48{\small $\pm$.48} \\ 
ProtoNet$^*$ & -&-&-&- & 73.29{\small $\pm$.71}  &79.72{\small $\pm$.79}    & 39.57{\small $\pm$.57} & 24.05{\small $\pm$1.01}\\
MetaOpt$^*$  & -&-&-&-& 64.44{\small $\pm$.73}  & 68.41{\small $\pm$.73}    & 36.28{\small $\pm$.50} & 22.53{\small $\pm$.91}\\
% \midrule
STARTUP$^\dagger$ & 63.88{\small $\pm$.84} & 75.93{\small $\pm$.80} & 32.66{\small $\pm$.60} & {23.09}{\small $\pm$.43}  &  82.29{\small $\pm$.60} & 93.02{\small $\pm$.45}  & 47.22{\small $\pm$.61}  & 26.94{\small $\pm$.45} \\
\midrule
ProtoNet &  55.32{\small $\pm$.88} &  52.94{\small $\pm$.81} &  29.58{\small $\pm$.57} &  21.32{\small $\pm$.37} 
&  76.92{\small $\pm$.67} &  81.84{\small $\pm$.68} &  42.49{\small $\pm$.58} &  24.72{\small $\pm$.43} \\
MatchingNet          &  54.88{\small $\pm$.90} &  46.86{\small $\pm$.88} &  27.37{\small $\pm$.51} &  20.65{\small $\pm$.29} 
&  68.00{\small $\pm$.68} &  63.94{\small $\pm$.84} &  33.96{\small $\pm$.54} &  22.62{\small $\pm$.36} \\
ce                   &  58.14{\small $\pm$.83} &  68.78{\small $\pm$.84} &  32.12{\small $\pm$.59} &  22.60{\small $\pm$.39} 
 &  80.09{\small $\pm$.61} &  89.79{\small $\pm$.52} &  43.88{\small $\pm$.57} &  26.51{\small $\pm$.43} \\
simclr               &  58.28{\small $\pm$.90} &  61.58{\small $\pm$.88} &  32.43{\small $\pm$.56} &  22.37{\small $\pm$.42} 
 &  80.83{\small $\pm$.64} &  83.44{\small $\pm$.61} &  44.04{\small $\pm$.55} &  26.63{\small $\pm$.46} \\
simclr-u             &  62.63{\small $\pm$.87} &  69.22{\small $\pm$.93} &  31.45{\small $\pm$.59} &  23.59{\small $\pm$.44} 
&  82.76{\small $\pm$.59} &  89.31{\small $\pm$.53} &  42.18{\small $\pm$.54} &  29.56{\small $\pm$.49} \\
startup              &  64.32{\small $\pm$.88} &  74.45{\small $\pm$.86} &  31.73{\small $\pm$.57} &  22.27{\small $\pm$.41} 
 &  83.58{\small $\pm$.60} &  92.41{\small $\pm$.47} &  45.73{\small $\pm$.62} &  26.21{\small $\pm$.46} \\
ce-simclr            &  63.91{\small $\pm$.83} &  70.35{\small $\pm$.85} &  31.67{\small $\pm$.55} &  23.72{\small $\pm$.44} 
&  85.78{\small $\pm$.51} &  91.10{\small $\pm$.49} &  45.97{\small $\pm$.54} &  30.23{\small $\pm$.50} \\
% ce-distill-fixed-sgd &  70.07{\small $\pm$.88} &  76.73{\small $\pm$.82} &  35.28{\small $\pm$.61} &  22.33{\small $\pm$.43} 
% &  86.35{\small $\pm$.52} &  93.20{\small $\pm$.42} &  49.34{\small $\pm$.60} &  26.30{\small $\pm$.45} \\
\rowcolor{Gray}
\Ours   &  71.62{\small $\pm$.84} &  81.52{\small $\pm$.78} &  34.08{\small $\pm$.58} &  23.03{\small $\pm$.43} 
  &  88.51{\small $\pm$.47} &  95.19{\small $\pm$.38} &  48.20{\small $\pm$.59} &  28.31{\small $\pm$.46} \\
\bottomrule
\hline
\end{tabular}


==> NeurIPS2021/Tables/main_tbl/results_res10_linear.tex <==
\begin{tabular}{lllll}
\toprule
{} & EuroSAT & CropDisease &   ISIC & ChestX \\
\midrule
ce                   &   92.07 &       95.37 &  76.39 &  44.13 \\
simclr               &   92.36 &       90.91 &  76.52 &  47.08 \\
simclr-u             &   93.22 &       95.27 &  76.42 &  48.04 \\
startup              &   93.84 &       97.29 &  77.46 &  44.96 \\
ce-simclr            &   93.77 &       96.35 &  76.07 &  47.53 \\
% ce-distill-fixed-sgd &   94.20 &       96.85 &  77.43 &  46.28 \\
ce-distill-ema-sgd   &   94.55 &       97.59 &  76.23 &  46.67 \\
\bottomrule
\end{tabular}


==> NeurIPS2021/Tables/main_tbl/tbl_ablation.tex <==

\begin{table}[ht]
\centering
\small
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{ cccc|c  c  c  c}

\hline
\toprule

\textbf{Momentum Teacher} & \textbf{Sharpening} & \textbf{Soft-threshold} & \textbf{Aug} &    EuroSAT &             CropDisease &                    ISIC &                  ChestX \\
\midrule
%  \xmark & \xmark & \xmark & \xmark                        
%  & 85.24 & 93.70 & 50.92 & 26.32 \\
 
  \cmark & \xmark & \xmark & \xmark                        
 & 84.95 & 93.50 & 50.70 & 26.24 \\
 
  \cmark & \cmark & \xmark & \xmark                        
 & 84.52 & 93.67 & 49.70 & 26.61 \\
 
  \cmark & \cmark & \xmark & \cmark                        
 & 88.89 & 95.65 & 49.95 & 28.31 \\
 
 
%  \xmark & \cmark & \cmark & \cmark                        
%  & 86.35 &       93.20 &  49.34 &  26.30 \\
%  \cmark & \cmark & \cmark &  \xmark
%  & 84.40 & 93.63 & 50.23 & 26.55 \\
%  & \cmark & \cmark &                   
% & & & & \\
%  & \cmark & \cmark &           
%  & & & & \\
%  &  &  &   & & & & \\
 
%  \cmark & \cmark & \cmark & \cmark &
%  88.51 & 95.19 & 48.20 & 28.31 \\
\bottomrule

\end{tabular}
\end{adjustbox}

\caption{\textbf{Ablation study on four benchmark datasets with ResNet-10 as backbone network in terms of 5-way 5-shot accuracy (\%).}  }
\label{table:ablation}
\end{table}

==> NeurIPS2021/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See supplementary}
% %   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
% %   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% % Please do not modify the questions and only use the provided macros for your
% % answers.  Note that the Checklist section does not count towards the page
% % limit.  In your paper, please delete this instructions block and only keep the
% % Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{\bf See Appendix}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{\bf See Sec.~\ref{sec:broader_impact}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{\bf See Sec. ~\ref{sec:exp}}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{\bf 95\% confidence intervals are provided for the main results}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{\bf See Appendix}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
   \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
   \answerNA{}
\end{enumerate}

\end{enumerate}
